Evidence for Environmental Dependence of the Upper Stellar Initial Mass Function in Orion A

We extend our previous study of the stellar population of L1641, the lower-density star-forming region of the Orion A cloud south of the dense Orion Nebula Cluster (ONC), with the goal of testing whether there is a statistically significant deficiency of high-mass stars in low-density regions. Previously, we compared the observed ratio of low-mass stars to high-mass stars with theoretical models of the stellar initial mass function (IMF) to infer a deficiency of the highest-mass stars in L1641. We expand our population study to identify the intermediate mass (late B to G) L1641 members in an attempt to make a more direct comparison with the mass function of the nearby ONC. The spectral type distribution and the K-band luminosity function of L1641 are similar to those of the ONC (Hillenbrand 1997; Muench et al. 2002), but problems of incompleteness and contamination prevent us from making a detailed test for differences. We limit our analysis to statistical tests of the ratio of high-mass to low-mass stars, which indicate a probability of only 3% that the ONC and the southern region of L1641 were drawn from the same population, supporting the hypothesis that the upper mass end of the IMF is dependent on environmental density.

==> KLF_list2.tex <==
\begin{deluxetable*}{c|c|c|c|c|c|c}
\small
\tablecaption{Number of Stars in K$_s$-magnitude Bins}

\tablehead{\colhead{Region}  & \colhead{$K_s < 7$} & \colhead{$7 < K_s < 8$} & \colhead{$8<K_s<9$} & \colhead{$9<K_s<10$} & \colhead{$10<K_s<11$} & \colhead{$11<K_s<12$}}
\startdata

ONC (\citet{Muench02})			&	8	&	10	&	29		&	82	&	132		&	183		\\	
\hline
L1641-all						&	4	&	10	&	23		&	51	&	139		& 	266		\\
							&		&		&	(+1)		&	(+5)	&	(+17)	&	(+40)	\\
\hline						
L1641-n						&	3	&	2	&	6		&	17	&	42		&	104		\\
							&		&		&			&	(+1)	&	(+3)		&	(+3)		\\
\hline
L1641-s						&	1	&	8	&	17		&	34	&	97		&	162		\\
							&		&		&	(+1)		&	(+4)	&	(+14)	&	(+37)	\\

\enddata	
\label{tab:KLF_list}
\end{deluxetable*}
